Precision measurement of the mass difference between light nuclei and anti-nuclei

The measurement of the mass differences for systems bound by the strong force has reached a very high precision with protons and anti-protons. The extension of such measurement from (anti-)baryons to (anti-)nuclei allows one to probe any difference in the interactions between nucleons and anti-nucleons encoded in the (anti-)nuclei masses. This force is a remnant of the underlying strong interaction among quarks and gluons and can be described by effective theories, but cannot yet be directly derived from quantum chromodynamics. Here we report a measurement of the difference between the ratios of the mass and charge of deuterons and anti-deuterons, and $^{3}{\rm He}$ and $^3\overline{\rm He}$ nuclei carried out with the ALICE (A Large Ion Collider Experiment) detector in Pb-Pb collisions at a centre-of-mass energy per nucleon pair of 2.76 TeV. Our direct measurement of the mass-over-charge differences confirm CPT invariance to an unprecedented precision in the sector of light nuclei. This fundamental symmetry of nature, which exchanges particles with anti-particles, implies that all physics laws are the same under the simultaneous reversal of charge(s) (charge conjugation C), reflection of spatial coordinates (parity transformation P) and time inversion (T).

==> sources/abstract.tex <==
The measurement of the mass differences for systems bound by the strong force
has reached a very high precision with protons and anti-protons\cite{pbarMass,TRAP}.
The extension of such measurement from (anti-)baryons to (anti-)nuclei allows one
to probe any difference in the interactions between nucleons and anti-nucleons encoded
in the (anti-)nuclei masses. This force is a remnant of the underlying strong interaction
among quarks and gluons and can be described by effective theories\cite{NuclForces},
but cannot yet be directly derived from quantum chromodynamics.
Here we report a measurement of the difference between the ratios
of the mass and charge of deuterons ($\bf{d}$) and anti-deuterons ($\bf{\bar{d}}$), and \Hebf and \Hebarbf
nuclei carried out with the ALICE (A Large Ion Collider Experiment)\cite{ALICE}
detector in Pb-Pb collisions at a centre-of-mass energy per nucleon pair of 2.76 TeV.
Our direct measurement of the mass-over-charge differences confirm CPT invariance
to an unprecedented precision in the sector of light nuclei\cite{CPTtheorem_1,CPTtheorem_2}.
This fundamental symmetry of nature, which exchanges particles with anti-particles,
implies that all physics laws are the same under the simultaneous reversal of charge(s) (charge conjugation C),
reflection of spatial coordinates (parity transformation P) and time inversion (T).

